OpinionConv: Conversational Product Search with Grounded Opinions

When searching for products, the opinions of others play an important role in making informed decisions. Subjective experiences about a product can be a valuable source of information. This is also true in sales conversations, where a customer and a sales assistant exchange facts and opinions about products. However, training an AI for such conversations is complicated by the fact that language models do not possess authentic opinions for their lack of real-world experience. We address this problem by leveraging product reviews as a rich source of product opinions to ground conversational AI in true subjective narratives. With OpinionConv, we develop the first conversational AI for simulating sales conversations. To validate the generated conversations, we conduct several user studies showing that the generated opinions are perceived as realistic. Our assessors also confirm the importance of opinions as an informative basis for decision-making.

==> SIGdial23-opinionConv-part5-discussion.tex <==
\section{Research Enabled By OpinionConv}

In this section, we introduce a few more examples of research problems in opinionated conversational product search that can be addressed using the new dataset generated by OpinionConv.\newline
\textbf{Opinionated Conversational Response Modeling:}
A key research task in multi-turn conversational product search is generating fluent and informative natural responses while maintaining representative internal states in each dialogue utterance for product search optimization. Since OpinionConv has control over both the structure of the dialogue and the incorporation of subjective narratives into the conversation, it enables the researchers and practitioners to conduct a detailed analysis of generation models from both customer and sales assistant perspectives. Therefore, the dataset generated by OpinionConv complements the existing datasets for conversational product search and can potentially impact the progress in this area of research significantly.
\newline
\textbf{Dialogue Response Selection:}
Since generated responses to both customer and sales assistant come from real product reviewers with different points of view about the features of products, the generated dataset by OpinionConv contains several dialogue pairs for a given question or opinion whose differences are the subjective narrative of reviewers. This, on the one hand, increases the diversity in the conversation utterances, and on the other hand, enables further study on dialogue response selection in opinionated conversational product search.
\newline
\textbf{Future Work:} An opinion is an observation or a belief that does not need to have evidence to support itself, whereas an argument requires reasons. As we showed in the evaluation, one of the improvements that study participants wanted to see was having stronger arguments in the generated conversation, rather than only expressing opinions. This enables researchers to study the argumentative dialogue systems in the conversational product search.

%This new dataset opens up a range of research opportunities in the fields of conversational opinionated question answering and (interactive) information retrieval for product search. Directions for future work include automatically training and developing conversational product search assistants as well as investigating argument mining techniques to assess the strength of opinions to improve the quality of the conversational dataset.

